Run-time Monitoring of 3D Object Detection in Automated Driving Systems Using Early Layer Neural Activation Patterns

Monitoring the integrity of object detection for errors within the perception module of automated driving systems (ADS) is paramount for ensuring safety. Despite recent advancements in deep neural network (DNN)-based object detectors, their susceptibility to detection errors, particularly in the less-explored realm of 3D object detection, remains a significant concern. State-of-the-art integrity monitoring (also known as introspection) mechanisms in 2D object detection mainly utilise the activation patterns in the final layer of the DNN-based detector's backbone. However, that may not sufficiently address the complexities and sparsity of data in 3D object detection. To this end, we conduct, in this article, an extensive investigation into the effects of activation patterns extracted from various layers of the backbone network for introspecting the operation of 3D object detectors. Through a comparative analysis using Kitti and NuScenes datasets with PointPillars and CenterPoint detectors, we demonstrate that using earlier layers' activation patterns enhances the error detection performance of the integrity monitoring system, yet increases computational complexity. To address the real-time operation requirements in ADS, we also introduce a novel introspection method that combines activation patterns from multiple layers of the detector's backbone and report its performance.

==> sec/6_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/oldtexint.tex <==
\section{Introduction}
For effective functioning across various driving scenarios,  perception plays a pivotal role, involving the sensing and understanding of the vehicle's environment. This task is fundamental as the entire automated driving system (ADS) architecture relies significantly on its environmental comprehension. The essence of the perception process lies in its capacity to precisely localise and categorise other road users and objects in the vicinity. Failure to do so can lead to dangerous and costly road accidents. For example, in \cite{eduardo1} and \cite{eduardo2}, the ADS's perception mechanism failed to accurately detect objects, leading to incidents that resulted in fatalities or severe injuries to the occupants. Such accidents highlight the critical need for perception systems to be resilient against the run-time errors that may arise, despite the efforts in design to minimise them. To ensure a fail-safe operation, ADS must be equipped with a tailored mechanism, to continuously monitor the perception system for potential errors \cite{hakansurvey,rahmansurvey}. Once such an error is detected, the next action is to issue an alert which can be used to hand over the control to the driver or trigger a minimum risk manoeuvre depending on the automation levels defined by SAE \cite{sae}.
%must trigger an alert. Depending on the level of autonomy, an alert can hand over the control back to the human driver in SAE level 3, or initiate a minimum risk manoeuvre in SAE level 4. % see Fig.~\ref{fig:overview}. 
\begin{figure}[t]
    \centering
    \includegraphics[width =\linewidth]{figs/graphabs2.png}
    \caption{\textbf{High level summary of the paper:} Main pipeline of LIDAR-based object detection is depicted at the top where a processor network extracts features and transforms point cloud first. This data then fed into a backbone network, which computes both mid-layer and last-layer neural activation patterns. These patterns are extracted and subsequently handled by the Neural Activation Pattern Operator, which either concatenates them (proposed mechanism) or selects one of the layers (earlier layer investigation). The chosen neural activation pattern is then inputted into the Introspection Network. The Introspection Network's output classifies the instance as either 'Error' or 'Not Error}
    \label{fig:overview}
\end{figure}

State-of-the-art (SOTA) object detection mechanisms usilise various types of  deep neural networks (DNNs) that have recently shown remarkable performance on various benchmarks~\cite{detectionsurvey,detectionsurvey2} and continue to be an active area of research for further improvement. Despite these advancements, object detectors in ADSs are not entirely free from errors especially in driving domain. This is due to the broad range of scenarios and complexity of many road users acting independently. To mitigate this issue and provide a remedy to such cases, a common method employed in ADSs is to develop a separate run-time monitoring mechanism to decide when to accept or reject perception outputs to ensure safety, which is also called by the term \textit{``introspection"} within the context of ADS.

In the recent literature, various methods for introspection in DNN-based systems have been explored, focusing on distinct input representations and techniques for identifying errors. One such method is based on confidence or uncertainty, utilising the output's certainty level for error detection as discussed in \cite{dropoutod}. Another strategy involves identifying discrepancies in multiple, varied parallel systems, exemplified by the comparison of detection and tracking in \cite{failingtolearn}. For ADS in controlled settings, using a history-based introspection approach shows promise. This method relies on the storage and retrieval of past experiences for error identification, as mentioned in \cite{fitforpurpose}. Additionally, assessing the maximum potential of performance metrics, like mean average precision (mAP), offers a way to pinpoint instances where system performance falls below a specific standard, as detailed in \cite{rahmanper}.


Despite gaining significant attention in the past decade, run-time monitoring of DNN-based mechanisms in ADS domain has centred on 2D object detection and classification functions \cite{hakansurvey}. However, as automated driving systems aspire to achieve higher levels of autonomy, they increasingly incorporate an additional array of sensors for robust object detection in adverse and variable conditions. Moreover, the inherently three-dimensional nature of the world requires a comprehensive understanding of the environment in 3D to ensure the resilience and robustness of ADS applications. Additionally, in recent years, investigating neural activation patterns for either uncertainty estimation, or for identifying performance drops, has gained popularity due to its flexibility and ease of integration into other systems \cite{rahmanper}. However, despite this popularity and the necessity for an investigation for the monitoring of commonly utilised LIDAR-based 3D object detection, only limited attempts made mainly around uncertainty estimation \cite{feng2018towards,feng2019can}. This motivates the investigation of utilising neural activation patterns for identifying performance drops, or scenes where false negative detections occur for LIDAR-based 3D object detection.


This research first assesses the applicability and effectiveness of advanced introspection mechanisms, particularly those that leverage neural activation patterns, in the realm of LIDAR-based 3D object detection. Subsequently, it investigates the impact of neural activation patterns from earlier layers as opposed to the traditional reliance on activations from the final layer. This exploration is founded on the hypothesis that, in contrast to camera-based 2D detection, the sparse nature of LIDAR data might render activations from the final layer insufficient for accurately identifying instances where the object detection model fails. Additionally, the study introduces a novel introspection approach that integrates neural activation patterns from multiple layers for better error detection. For this purpose, we utilise the widely used baseline models PointPillars\cite{pointpillars} and CenterPoint\cite{centerpoint}, and extract neural network activation patterns from multiple layers of its backbone model, SECOND \cite{SECOND}. The errors are labelled if the object detector is missed an actor, and the (binary) labels are paired with the raw neural activation patterns. Subsequently, an introspector convolutional neural network (CNN) is trained on the generated pairs, hereafter referred to as the error dataset. A high-level summary of our mechanism is presented in \Cref{fig:graphicalabs}.
In summary, the contributions of this paper are:
\begin{itemize}
    \item Comprehensive assessment of advanced introspection mechanisms utilising neural activation patterns in LIDAR-based 3D object detection.
    \item Investigation into the efficacy of extracting neural activation patterns from earlier layers versus traditional reliance on final layer activations, especially in the context of LIDAR's sparse data nature compared to camera-based 2D detection.
    \item Introduction of a novel introspection approach integrating neural activation patterns from multiple layers for enhanced error detection in 3D object detection models.
    \item Qualitative and quantitative evaluation of the adapted mechanisms, earlier neural activation patterns and proposed mechanism in terms of error detection capability on two well-known public driving datasets, KITTI~\cite{kitti} and NuScenes~\cite{nuscenes}, and widely used object 3d object detector baselines in ADS, PointPillars~\cite{pointpillars} and CenterPoint~\cite{centerpoint}.

\end{itemize}

The structure for the rest of this paper is as follows: In \Cref{sec:litr}, we review the current literature on introspection of object detection. \Cref{sec:meth} outlines the adapted mechanism and introspection method proposed. Experimental settings and performance evaluation is presented in \Cref{sec:perfeval}. Finally, key takeaways of the papers are given in \Cref{sec:conc}.
%proposes a novel introspection method for LIDAR-based 3D object detection in ADSs by utilising multi-layer neural network activation patterns. Our study focuses on LIDAR-based 3D object detection as it is the most common sensor modality for 3D object detection unless multi-modal solutions are employed. In addition, to ensure a fair comparison and comprehensively evaluate the performance of the proposed method, we adapted the different mechanisms proposed for introspection of 2D object detection to conduct comparative analysis between our solution and the adapted mechanisms.
% \label{sec:intro}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

